Sources of Uncertainty in Supervised Machine Learning -- A Statisticians' View

Supervised machine learning and predictive models have achieved an impressive standard today, enabling us to answer questions that were inconceivable a few years ago. Besides these successes, it becomes clear, that beyond pure prediction, which is the primary strength of most supervised machine learning algorithms, the quantification of uncertainty is relevant and necessary as well. However, before quantification is possible, types and sources of uncertainty need to be defined precisely. While first concepts and ideas in this direction have emerged in recent years, this paper adopts a conceptual, basic science perspective and examines possible sources of uncertainty. By adopting the viewpoint of a statistician, we discuss the concepts of aleatoric and epistemic uncertainty, which are more commonly associated with machine learning. The paper aims to formalize the two types of uncertainty and demonstrates that sources of uncertainty are miscellaneous and can not always be decomposed into aleatoric and epistemic. Drawing parallels between statistical concepts and uncertainty in machine learning, we emphasise the role of data and their influence on uncertainty.

==> 3-Sources/ensembles.tex <==
\subsection{Ensemble Methods and Stochastic Algorithms}
{\color{red}[CG: What are we trying to say with this part?]}\\
{\color{green}[]GK: Finde ich gar nicht schlecht, dass wir auch etwas über Ensemble oder besser algorithmische Unsicherheit liefern]}
\cg{Ensembles are one way how to quantify uncertainty, but so are Bayesian methods  (and everything else Eyke mentioned in \cite{hullermeier2021AleatoricEpistemicUncertainty}). I think we should not selectively introduce some quantification methods.}
We defined with $\hat{p}_{Y|X}(\cdot|x) $ the trained model, learned based on data ${\cal D}$ using some algorithm ${\cal A}$. 
The latter itself can be random due to some random initialisation or random components, e.g. stochastic gradients. In fact, the above mentioned regularization for overparameterized models can also be induced by stochastic components, as indicated by the prior. This in turn means that even the prediction model can be random if it is based, for instance, on a random ensemble. We refer to \citet{neal2018ModernTakeBiasVariance}.....
\textcolor{brown}{\\PS:
\begin{enumerate}
    \item I hope it's not just semantics, but there's a difference between the general, abstract  algorithm ${\cal A}$ and the trained algorithm or trained prediction model (having been fed these specific data and having been trained). Most, if not all, prediction models are not random anymore: if you feed a specific input 1000 times, 1000 times you will get the exact same prediction value output. but some algorithms can even make random decisions (think of randomisierte Tests), although this might be more relevant for decision-making algorithms (e.g., ADMs) than for simple prediction models.
    Or, in other words: there's randomness that can produces different values for $\hat{\theta}$ from the very same data. But there's also randomness, that, for fixed data and fixed $\hat{\theta}$, can produce different values of $\hat{y}$ for the same input $x_{new}$. These 2 randomnesses are not the same.
    \item Related: can we say something about the different between algorithm and model class? Some may think that, e.g., OLS regression is both an algorithm and a model class, there's no difference?
    \item Wouldn't it be great if we had a relatively long list of these types of random aspects of algorithms? Or is this what \citet{neal2018ModernTakeBiasVariance} produces? Maybe it's also informative for our thinking if we list these components here?
    \item Can explicitly say something about the relationship between a prediction model (class) and the algorithm? Something along the lines of the following (hope, I'm not wrong): For some prediction model classes, there exists more than one possible algorithm for implementation. Hence, we want to make explicit the model was trained using algorithm ${\cal A}$ specifically by including it as a subscript.
    \item Also: how does the choice of a loss function figure into this? Is this part of the algorithm? If not, then maybe it's worth including elsewhere: uncertainty about which loss function to choose translates to uncertainty about the final model (but ``invisibly'' so).
    \item I don't know what a random ensemble is. Include short explanation + reference?
    \item right now, there's only a brief mention of ensembles. should the subsection's title then really include and start with ``ensemble methods''?
\end{enumerate}}


We therefore include the algorithm itself in the prediction model and write $\hat{\theta}_{({\cal A})}$ for the trained parameter, based on algorithm ${\cal A}$.  The average run of the algorithm then provides the fitted model through
\begin{align*}
  \hat{p}_{Y|X}(\cdot | x) := E_{{\cal A}}\left(p_{Y|X}(\cdot|x ; \hat{\theta}_{({\cal A}))}\right)
\end{align*}
where the expectation is taken with respect to the stochastic components of the algorithm.  Correspondingly we define with
\begin{align*}
\mbox{Var}_{{\cal A}} \left(\hat{p}_{Y|X}(\cdot|x )\right)
& =  E_{{\cal A}} \left( \left\{p_{Y|X}(\cdot|x ; 
\hat{\theta}_{({\cal A})} - \hat{p}_{Y|X}(\cdot|x) \right\}^2 \right)
\end{align*}
the variance resulting through the stochasticity in the algorithm. Note that this variance is zero for deterministic algorithms, i.e.\ algorithms that for given data will always lead to the same estimate. We define the resulting uncertainty as {\sl algorithm uncertainty}, which generally should be small compared to the above uncertainties. If the algorithm is only run once we take $\hat{p}_{Y|X}(\cdot|X) = p_{Y|X}(\cdot | x, \hat{\theta}_{({\cal A})})$, but in this case we can neither estimate nor assess the algorithmic uncertainty. Apparently, in overparameterized models such as deep learning it may be numerically very demanding to train the model  multiple times, which expresses due to the necessity of regularization the influence of stochastic version for regularization. (TO BE CONTINUED)



{\color{green}{That needs more discussion, since in deep learning this becomes an issue}}
{\color{red}{GK: Hier sollte man auch noch etwas zu den random dropout von Gewichten schreiben. Denn das wird ja Bayesianisch motiviert}}


\textcolor{brown}{PS:
\begin{enumerate}
    \item we used curly braces $\left\lbrace \right\rbrace$ for the expected values $E$ earlier on, but here it's big round parentheses. I think consistency would help the reader.\\
    conversely, the curly braces in the 2nd equation probably should round parentheses?
    \item I like the idea of $E_{{\cal A}}$! But some algorithms can fail to produce a result, e.g., they do not converge. What then? Does that mean that expected value does not exist? And, more practically, what to do then w/ the mean. A-L Boulesteix recently had something on this, but I don't know if it's published yet. (It was more about simulations, I think, but still: what to do w/ runs fail. ignore, impute, ... ?)
    \item on ``{\sl algorithm uncertainty}, which generally should be small compared to the above uncertainties'': what does ``should'' mean? That this is true in most cases or that it better be true or we're in trouble? don't know if we can say this w/o further clarification or references. I think some things, like clustering, can be very unstable and susceptible.
    \item on ``If the algorithm is only run once we take $\hat{p}_{Y|X}(\cdot|X) = p_{Y|X}(\cdot | x, \hat{\theta}_{({\cal A})})$, but in this case we can neither estimate nor assess the algorithmic uncertainty'': what's the difference between estimate and assess?
    \item the last sentence is not quite finished yet, I think.
\end{enumerate}
}


==> 3-Sources/overparam-short.tex <==
\subsection{Overparameterized Models, Deep Learning and Double Descent}
\label{sec:overparameterized-short}

\cg{shortened version needs refinement}
We want to get a little deeper into the classical bias-variance tradeoff but focus on \textit{overparameterized} models, as they are typical in deep learning. 
This means that the dimension of the parameter set exceeds the number of observations $n$.  


Traditionally, statistical setups assume $p < n$ with $n$ as the sample size. Recent literature focuses on model performance if in contrast $p > n$,
see for instance \citet{efron2020prediction},
\citet{fan2021selective}, \citet{bartlett2021deep} or \citet{hastie2022surprises}, to name but a few. In fact, the success of deep learning is based on heavily overparameterized models which utilize the fact that a second bias-variance trade-off optimum, can occur in constellations with more parameters than observations. This phenomenon is also known as \textit{double descent} \citep{belkin2019ReconcilingModernMachinelearning, neal2018ModernTakeBiasVariance, neyshabur2018UnderstandingRoleOverParametrization, yang2020RethinkingBiasvarianceTradeoff, zhang2021UnderstandingDeepLearning}. 
In the overparameterized model it is however required to regularize the estimation. In statistical terminology this is known as penalization or ridging, which in fact corresponds to imposing a prior distribution on the parameter in a Bayesian style, see e.g. \citet{fortuin2022priors} or \citet{wang2020survey}.
We want to look at the case $p>n$ in more depth now.

[......]
Compared with equation (\ref{eq:decomposition.of.prediction.error}), just like ${bias}( \hat{y} |x)^2$, the first component describes discrepancies between the true model and the optimal estimate (model uncertainty). The second component mirrors ${Var}(\hat{y}|x)$ in that it measures how much the fitted models will, on average, deviate from the optimal one (estimation uncertainty).  With increasing dimension of $\theta$, the first component gets smaller, since the difference, and hence the Kullback-Leibler divergence between the true distribution $f(y|x)$ and the optimal $p(y|x;\theta_0)$, gets smaller. The second component in contrast can get larger since the regularization increases the bias of the estimate $\hat{\theta}_{pen}$. We provide more explanations in  Appendix~\ref{Appendix:KL1}. This, in turn, mirrors the classical behaviour of the Kullback-Leibler divergence, utilized for instance in the AIC. However, we are here in the setup where $p>n$, which the AIC does not cover.  This property can lead to the fact, that for $p>n$ we find a second (local) minimum in the Kullback-Leibler divergence, namely one for $p<n$ and another one for $p>n$, where the latter heavily depends on the regularization/prior used to obtain a maximum of (\ref{eq:penlik}).


We can conclude that model selection based on minimizing the Kullback-Leibler divergence between the ``true'' model and the model class ${\cal P}$ extends towards overparameterized models, where regularization needs to be taken into account for estimation. This can lead to selected models with more parameters than observations, a finding which is not yet completely established and understood in statistics. 


==> 4-deficient-data-model-uncertainty/conntecting-tse-to-alea-epist.tex <==
\subsection*{Connection to Aleatoric and Epistemic Uncertainty}     \label{subsec:connecting.tse.to.chapter.2}

\alert{to do}: da einbauen, wo es hin soll.\\
again a matter of perspective/context what is or is not aleatoric. outcome | features: but do we mean true values or error-prone values? setting aside the design aspect: it's also about whether we model the error (ME; annotator contributions) -- if so, there's epistemic uncertainty stemming from the correction model's uncertainty.

==> 4-deficient-data-model-uncertainty/errors-in-x-old.tex <==

\highlight{Status:}  \textit{Mittelfristig:\\
1. evtl. SIMEX Anwendung zeigen (siehe Anmerkung im Text).\\
2. Ich frage mich, ob man diese subsection a) noch ueberzeugender machen kann z.B. mit Simulationen wie im Omitted Variable Kapitel oder ob b) noch mehr Bezug zu Uncertainty und UQ herstellbar ist.} 

\paragraph{Terminology}
%\textcolor{blue}{neue Version (ich kann nicht den ganzen Abschnitt mit den TeX-Befehlen blau machen, darum manuell drüber geschrieben:\\}
In the pertinent literature, the term \emph{measurement error} (ME) commonly refers only to errors in the features and not to errors in $Y$ (section~\ref{subsec:errors.in.y}). In addition, \emph{measurement error} can have two meanings: first, as an umbrella term encompassing errors in all types of features -- continuous, categorical, etc. -- and, second, to specifically denote errors in continuous features \citep[ch.~2]{keogh.et.al.2020.stratos.measurement.error.1}.\footnote{
	\emph{Misclassification} is employed to make explicit that an error-prone feature is categorical \citep[ch.~2.2.7]{carroll.et.al.2006.measurement.error}. Again, the error is solely in the features and not in $Y$, even if the term \emph{misclassification} used in the measurement error literature might feel misleading.
} 

Within the TSE framework above, \emph{measurement error} was a specific component situated between measurement instrument and response. It is unfortunate that the same term is used for different concepts. The errors that we consider in this subsection and the next subsection (errors in $Y$) can occur during the measurement (i.e., what the TSE would call measurement error) but also during labelling or processing. For the rest of this subsection, \ref{subsubsec:errors.in.x}, we will not use the term measurement error in TSE sense again.

%\textcolor{red}{alte Version:\\}
%In contrast to the previous subsection, \ref{subsubsec:errors.in.y}, we now consider what is called \emph{measurement error} (ME) in the pertinent statistical literature: errors being present in the features $X$, but not in $Y$. More specifically, \emph{measurement error} is a term used in two different ways: first, as an umbrella term encompassing errors in all types of features -- continuous, categorical, etc. -- and, second, to specifically denote errors in continuous features \citep[ch.~2]{keogh.et.al.2020.stratos.measurement.error.1}.\footnote{
%	\emph{Misclassification} is employed to make explicit that an error-prone feature is categorical \citep[ch.~2.2.7]{carroll.et.al.2006.measurement.error}. Again, the error is solely in the features and not in $Y$, even if the term \emph{misclassification} used in the ME literature might feel misleading.
%} 



\paragraph{Consequences}
The ``triple whammy of measurement error'' \citep[p.~1]{carroll.et.al.2006.measurement.error} comprises masking of some of the data's properties, loss of power to detect relationships (among the features and of the features to the outcome variable), and biased parameter estimates. The first two of these impacts make it more difficult to understand, diagnose, and hence develop a model: visual inspection and feature engineering, whether manual or automatic, are impaired; so are diagnosis-based changes to the model due to, e.g., miscalibration or other undesirable behaviours.\footnote{ 
    Uncertainty quantification is not limited to predictions. E.g., explanations given by interpretable machine learning \citep{molnar.2020.interpretable.ml} are also accompanied by uncertainty quantifications -- and these are affected by data deficiencies such as measurement error. 
} 
We elaborate a bit more on the third of these issues: bias.

%Let the $j$-th feature be subject to ME and let $X_j$ denote the observed, error-prone version of said feature while the unobserved, error-free variable $Z_j$ represents the true values. For simplicity, let all other features $X_{-j}$ be error-free, i.e., $X_i = Z_i$ for all $i \neq j$. We will focus on one such feature, $X_k = Z_k$, that is correlated with $Z_j$ and assume that all other features in $\mathbf{X_{-j}}$ are independent of $Z_j$.
Let $X_j$ denote the observed, potentially error-prone version of the $j$-th variable and the unobserved, error-free variable $Z_j$ denote corresponding true values.\footnote{
	We continue with our notation using $Y$, $X$, and $Z$ as introduced above. The notations used in the measurement error literature differ from ours.
}
Measurement error mechanisms, formalised as \emph{measurement error models}, can be of different types and can be quite complex. As the consequences are drastic even for simple and seemingly benign error mechanisms, we shall use a basic example to make the discussion more accessible. For a continuous feature, such a mechanism can be the so-called \emph{classical measurement error model}, 
\begin{align}
	X_j = Z_j + e_j \,\,\text{ with }\mathbb{E}(e_j|z_j) = 0 \text{ and } Var(e_j|z_j)=\sigma^2_j = const.\, \forall z_j.
	\label{eq:measurement.error.mechnism.example}
\end{align}


%a linear ME model,
%\begin{align}
%	X_j = \gamma_0 + \gamma_j Z_j + e,
%	\label{eq:measurement.error.mechnism.example}
%\end{align}
%and \highlight{check} we will consider the benign case where the error $e$ is independent from all components in $\mathbf{Z}$.

As much of the treatment of measurement error has focused on regression models (including generalised linear models such as logistic regression for non-continuous outcomes), %PS: das habe ich eingefügt, um klar zu machen, dass auch Regressionsmodelle zur Klassifikation untersucht wurden, sprich um das eventuelle ML-Missverständnis "Regression = stetige Variable" vorzubeugen, aber ist auch nicht so dramatisch wichtig. CG: dann evtl nur sagen: (including binary regression models)
let us use a linear model for sake of clarity. We will consider two variables that are subject to measurement error, $Z_1$ and $Z_2$, and an error-free variable $Z_3$, i.e., $Z_3 = X_3$, which may or may not be correlated with $Z_1$ and $Z_2$. %\footnote{
%    We could add other error-free features, ${X_4}={Z_4}$ and assume them to be independent of all errors and of $Z_1, Z_2, Z_3$ so that nothing happens to their beta coefficients. This would render our example closer to the usual ML set-up of many features, but it would only complicate our notation without additional insight.
%} 
Let the true relationship be
\begin{align}
	% Y = \beta_0 +  X_j \cdot \beta_j + \mathbf{X_{-j}} \cdot  \mathbf{\beta_{-j}} + \epsilon,
	Y = \beta_0 +  \beta_1 Z_1 + \beta_2 Z_2 +  \beta_3 Z_3 + \epsilon, \quad \epsilon \sim N(0, \sigma_{\epsilon}^2).
%	\label{eq:measurement.error.lin.model.true}
\end{align}
%The researcher would like to estimate the parameters of $Y | Z_1, Z_2, Z_3$, but 
The naive regression, ignoring the measurement error, estimates
\begin{align}
	% Y = \beta_0 +  X_j \cdot \beta_j + \mathbf{X_{-j}} \cdot  \mathbf{\beta_{-j}} + \epsilon,
    Y = \tilde{\beta}_0 +  \tilde{\beta}_1 X_1 + \tilde{\beta}_2 X_2 +  \tilde{\beta}_3 X_3 + \tilde{\epsilon}.
	\label{eq:measurement.error.lin.model}
\end{align}
%whose parameters are of interest to a researcher. Relative to the desired situation where in \eqref{eq:measurement.error.lin.model} we had the truth, $Z_j$, in place of the observed $X_j$, i.e., where we could learn
%\begin{align}
%	Y = \mathbf{Z}\cdot \mathbf{\beta} + \epsilon,
%	\tag{\ref*{eq:measurement.error.lin.model}$^\prime$}
%	\label{eq:measurement.error.lin.model.true}
%\end{align}% $Y = \mathbf{Z}\cdot \mathbf{\beta} + \epsilon$ 
In general, the consequences of measurement error include that $\hat{\tilde{\beta}}_0$, $\hat{\tilde{\beta}}_1$, $\hat{\tilde{\beta}}_2$, $\hat{\tilde{\beta}}_3$, and $\hat{\tilde{\sigma}}^2_{\epsilon}%= \hat{{Var}}(\epsilon|\mathbf{X})
$ are all biased for their counterparts from \eqref{eq:measurement.error.lin.model.true}. The direction and magnitude of the biases of the beta coefficients are unknown ex ante: they may be under- or overestimated, possibly even with the incorrect sign, and the magnitude can be large.\footnote{
    It is important to emphasise these results as, in our experience, unfortunately the intuition of many, even experienced researchers is 1) that measurement error in $X_j$ would only affect $\hat{\beta}_j$ but %\replace{no other weights}
    {none of the other beta coefficients} and 2) that the bias would always be one of attenuation, i.e., a bias towards zero. Both are decidedly not the case.
} 
A full discussion of the effects is beyond our scope. The main intuition is that the effects of variables with (high) measurement error is attributed to the features with no (or lower) measurement error. There are strong similarities to the situation of omitted variables \ref{subsubsec:omitted.variables}: 
as the amount of measurement error in feature $X_j$ increases, i.e., as $\sigma^2_j$ grows, the signal-to-noise ratio in $X_j$ decreases and the effect of $Z_j$ on $Y$ is increasingly picked up by other features to the extent that they are correlated with $Z_j$. In the limit, i.e., as $\sigma^2_j \to \infty$, 
$Y$ grows more and more independent from $X_j$ and the measurement error situation approaches an analogous setup of $Z_j$ being an omitted variable. The results from section~\ref{subsubsec:omitted.variables} on omitted variables thus apply here, too, and we do not repeat them.\footnote{
	It may be less obvious from the similarity to the omitted variables situation what happens with $\hat{\tilde{\beta}}_1$ and $\hat{\tilde{\beta}}_2$. This depends, e.g., on the correlation between $Z_1$ and $Z_2$ and the correlation among the errors, $e_1$ and $e_2$. Over- and underestimation and sign reversal are all possible even in simple scenarios.
}


%\begin{enumerate}
%	\item $\hat{\beta_j}$ is biased:
%	\item Other features are affected as well:
%	If another feature, $X_k$ is correlated with the error-prone $X_j$,\footnote{
%	$X_k$ and $X_j$ can be correlated because the true values, $Z_k$ and $Z_j$, are correlated or because $X_k$ is correlated with $e$, the error of $X_j$.	
%} 
%then its coefficient $\beta_k$ is also estimated with bias. 
%	\item $\hat{\sigma}^2 = \hat{Var}(\epsilon|...)$ is biased. hence prediction intervals or other measures of uncertainty are biased.
%\end{enumerate}

%The main intuition is the following. As the amount of measurement error in feature $X_j$ increases, i.e., as $\sigma^2_j$ grows, the signal-to-noise ratio in $X_j$ decreases. As a consequence, the effect of $Z_j$ on $Y$ is increasingly picked up by other features to the extent that they are correlated with $Z_j$. Whether this results in over- or underestimation depends on whether the features are positively or negatively correlated and on whether their effects on $Y$ are positive or negative. In the limit, i.e., as $\sigma^2_j \to \infty$, the measurement error setup approaches the situation of $Z_j$ being a an omitted variable \ref{subsubsec:omitted.variables}.

Several types of measurement error correction models have been developed. They build on an error mechanism such as \eqref{eq:measurement.error.mechnism.example}, estimate its parameters\footnote{
    In our example of the classical measurement error model \eqref{eq:measurement.error.mechnism.example}, $\sigma_j^2$ is the only parameter.
} 
from data or import the parameter values from external, auxiliary sources,\footnote{
	The data analyst must then decide whether these results are transportable to their training data (see \ref{subsec:distribution.shift} for more on transportability in general).
} 
and are then able to produce \emph{unbiased} estimates for the parameters of interest of the model for $Y | Z$. In order to estimate the parameters of the measurement error model, it is best to have some data that contain both, the error-prone $X_j$ and the error-free $Z_j$, for some instances.
%The appropriate data for estimating the parameters of the measurement error model usually require having both, the error-prone $X_j$ and the error-free $Z_j$, available for the same instances.
% This requires appropriate data.\footnote{
%	This typically takes one of two forms. Either for a subset in our training data, both $X_j$ and $Z_j$ are available so that the one can estimate the parameters of the measurement error model. %: in our example of the classical measurement error model \eqref{eq:measurement.error.mechnism.example}, $\sigma_j^2$ is the only parameter.
%	Or there are outside auxiliary data about the measurement error mechanism that produce the required knowledge about the measurement error model and its parameters. The data analyst must then decide whether these results are transportable to their training data (see \pageref{subsec:distribution.shift} for more on transportability in general).
%}

%\highlight{work in progress below}
%\add{eingefuegt: nachfolgend bis zum Abschnitt \textit{Fairness}}
While the measurement error literature has long progressed far past linear regression and has extended into, e.g., generalised linear models and nonlinear regression \citep{carroll.et.al.2006.measurement.error}, our presentation might still leave the impression that the topic is only of relevant to traditional statistical methods or when the interest is on the estimation of parameters. That is not the case; the linear regression case simply allowed us to convey concepts and results in the precise language of simple mathematics. However, there is still research to be done for extending measurement error concepts to machine learning and prediction-focused tasks. We already presented some of the consequences for predictive uncertainties above. We continue below. 

First, \citet[ch.~3.5]{carroll.et.al.2006.measurement.error} discuss the bias-variance trade-off \replace{from}{when} \cg{wrong preposition?}\pat{besser?} correcting for measurement error. To the best of the authors' and of our knowledge, this has been hardly explored in the literature. \cg{phrasing?}\pat{geaendert.} The authors use a single tuning parameter and show that the optimal level of measurement error correction is in general between 0 and 1, i.e., between no and full implementation of measurement error correction. \cg{Idea: either describe error correction procedure in more detail, or remove this part, as describing only the hyperparameter does not help understanding.} \pat{ich finde, dass das intuitive Verstaendnis hier ausreicht und eine laengere Behandlung keine Zusatzeinsicht bringt.}

Second, \citet{blackwell.et.al.2017.unified.measurement.error.missing.data.multiple.overimputation} present a unified approach, based on multiple imputation, that can correct for both, missing data (specifically: missing {cell}s %\cg{again: rather "cell"? like in an excel cell} 
or \emph{item nonresponse}, see section~\ref{subsec:missing.data}) and measurement error among some instances. Such general methods are very attractive for practical application as there may often be more than one type of deficiency in one's data. Here, the underlying methodology, multiple imputation, also allows the quantification of uncertainty to separate the part that is due to the data deficiency (measurement error or missingness) from the rest.

Finally, there are also less (or even non-)parametric measurement error correction models approaches. E.g., Simulation-Extrapolation or SIMEX (see \citealp[ch.~5]{carroll.et.al.2006.measurement.error}) notices that while one cannot take out measurement error, one can add more of it voluntarily. In our example \eqref{eq:measurement.error.mechnism.example}, this would mean increase to $Var(e_j)$ from $1 \cdot \sigma^2_j$ stepwise: e.g., for each of $1.25 \cdot \sigma^2_j, 1.5 \cdot \sigma^2_j, 1.75 \cdot \sigma^2_j, \ldots, 5 \cdot \sigma^2_j$, one creates synthetic data by adding more measurement error to the original data. This then produces a functional relationship of the estimated betas and the measurement error variance. The insight of SIMEX is to estimate this functional relationship and then extrapolate it back to the %desirable but unattainable 
point of $Var(e_j) = 0 \cdot \sigma^2_j$ to obtain an estimate for the unbiased betas. In prediction, we are not interested in those betas, but we may analogously try to use SIMEX to look at, e.g., how predictive accuracy or other measures of uncertainty change with the level of measurement error.\footnote{
    This may seem like a lot of work for high-dimensional prediction if many features are error-prone: however, if we are only interested in prediction instead of parameters, we are free to focus only on the most important features \citep[ch.~8.5]{molnar.2020.interpretable.ml}. 

    As it will still typically involve a complete re-training of the model, the approach may still be computationally prohibitive for extremely costly model classes.
} 
We are not aware of such attempts in the literature so far. \highlight{idealerweise:} \textit{kleine Simulation, die zeigt, dass es funktioniert, in Appendix packen, im Text 2-4 Saetze dazu schreiben. Wenn das zu tief einsteigt, in kleines Mini-Paper auslagern.}

% \cg{[kein neuer Kommentar] connection to machine learning and uncertainty? oftentimes the coefficients are of no interest in supervised ML.} 
%\subsubsection*{Why care as a Data Scientist?}
%\pat{war vorher Teil von \ref{subsubsec:errors.in.x}}


%\begin{align}
%	\mathbb{E}(\hat{\beta}_{included}) = \beta_{included} + 
%	\alpha_{omitted|included} \cdot \beta_{omitted} .
%	\label{eq:omitted.variable.bias}
%\end{align}
%\citep[ch.~3.4.1]{fahrmeir.et.al.2022.regression}


% Fairness: raus und verschoben in fairness.tex


==> 4-deficient-data-model-uncertainty/omitted-vars-cutted.tex <==
Second, assume now that the the marginal effect of $X$ is the same in the full and in the omitted variable model. Probably the most intuitive situation is that, in addition to $\frac{\partial E(Y|x,z)}{\partial x}$ being independent of $Z$, also $X$ and $Z$ are independent so that $\frac{\partial f_{Z|X}(z|x)}{\partial x} = 0$ and the second integral on the right-hand side of \eqref{eq:expmissingz} vanishes. 
%We see that if $\partial E(Y|x,z)/(\partial x)$ for given $x$ and $z$ \replace{depends on the value of $z$}{does not depend on the value of $z$} and  $X$ and $Z$  are independent, \add{i.e.,} $\partial f_{Z|X}(z|x) / \partial x = 0$, then \replace{the omitted variable $Z$ does not have an influence on the modelling of the mean}{the derivative remains the same regardless of whether $z$ was used for training or not} \ms{Is this what you intended to say?}. \pat{Ich stimme Malte zu. Das ist Szenario a/b: die Regressionslinien sind parallel verschoben, aber der marginale Effekt von $X$ auf $Y$ ist für alle Werte $z$ derselbe. Der konditionale mean ist dann sehr wohl von der omission von $Z$ betroffen, aber der marginale Effekt ist derselbe. Diese Situation zu betrachten bedeutet, eine deutlich beschraenkende Annahme zu treffen - und selbst in dieser Situation kommt es dann zu den Auswirkungen, die wir spaeter beschreiben. Das ist fuer mich einer der beiden Gruende, warum wir ueberhaupt den marginalen Effekt von $X$ auf $Y$ bei prediction-focused machine learning sprechen wuerden?}
%\pat{Irgendwas stimmt fuer mich hier entweder mit der Mathe oder der Notation (falls ja, dann vermutlich bzgl. den Erw.werten) von \eqref{eq:expmissingz} nicht. Denn: man nehme an, dass das das zweite nicht zutrifft, das erste aber schon. Wenn das erste zutrifft, also $\partial E(Y|x,z)/(\partial x) = const$ für alle $z$, dann $\partial E(Y|x,z)/(\partial x) = \partial E(Y|x)/(\partial x)$ und ich kann den Term vor das Integral ziehen, und das Integral über die Dichte wird zu 1. Dann steht da:}
%\begin{align}
%    \frac{\partial E(Y|x)}{\partial x} 
%       & = \frac{\partial E(Y|x)}{\partial x} +  \underbrace{\int_{z \in {\cal Z}} E(Y | x, z) \frac{\partial f_{Z|X}(z|x)}{\partial x} \: dz}_{\neq 0},
%       \notag
%\end{align}
%\pat{also sowas wie $g(x)=g(x)+h(x)$ mit $h(x) \neq 0$.}

However, even when we make this limiting assumption and thus make the full and the omitted variable model more similar, we still find increased uncertainty. This becomes obvious through the calculation of the variance: 
\begin{align}
\nonumber
    Var(Y|x) & =    
  \int_{z \in {\cal Z}}  Var(Y| x, z)   f_{Z|X}(z|x) \: dz \\
\label{eq:varincrease}
  & +  \int_{z \in {\cal Z}}
  \left(E(Y|x,z) - E(Y|x)\right)^2 f_{Z|X}(z|x) dz.
\end{align}
From (\ref{eq:varincrease}) we can easily read the property, that the variance increases, and hence the aleatoric uncertainty increases, if input variables are omitted. 
\pat{1. sehe ich das  postulierte Ergebnis " we still find increased uncertainty" an der Formel nicht. ich will doch $Var(Y|x)$ mit $Var(Y|x,z)$ vergleichen und der Vergleich wird nicht direkt vollzogen. Ich habe auch ein Gegenbeispiel, das zeigt, dass es nicht stimmt, dass immer $Var(Y|x,z) \leq Var(Y|x) \, \forall x, z$:\\
Sei $Z \in \lbrace 0, 1 \rbrace$ binär. Der Erwartungswert von $Y$ sei unabhängig von $Z$, aber die Varianz nicht:  $v_1 \coloneqq Var(Y|x,z=1) > v_0 \coloneqq Var(Y|x,z=0)$. Ein schönes Beispiel dazu: der wahre Zusammenhang ist linear. $E(Y|X,Z) = \alpha + \beta X$, sprich: wir haben zwei Regressionsgeraden, die genau aufeinander liegen. Die Punkte, die zu $Z=1$ gehören, streuen mehr als die Punkte, zu $Z=0$ gehören, um die Regressionsgerade. Wegen $E(Y|x,z) = E(Y|x) , \forall x,z$ ist der zweite Term auf der rechten Seite von \eqref{eq:varincrease} Null. Damit ist dann nur noch der erste Term übrig. Ich verwende nur die o.g. Definitionen und Annahmen und zähle in der 2. Zeile Null hinzu mit $0 = v_1 - v_1$:
\begin{align*}
    Var(Y|x) & = v_1 \cdot \Prob(Z=1|x) & + &  v_0 \cdot  \Prob(Z=0|x)\\
             & = v_1 \cdot \Prob(Z=1|x) & + &  (v_0 + v_1 - v_1) \cdot \Prob(Z=0|x) \\
             & = v_1 \cdot  \underbrace{(\Prob(Z=1|x) + \Prob(Z=0|x))}_{=1}            & + & \underbrace{(v_0 - v_1)}_{<0} \cdot \Prob(Z=0|x), 
\end{align*}
mithin ist für $z=1$ die Varianz $v_1 = Var(Y|x) \underbrace{-(v_0 - v_1) \cdot \Prob(Z=0|x)}_{>0}$ also größer als die Varianz von $Y|x$. Das Ergebnis hängt auch nicht dran, dass $Z$ binär ist; ich habe auch einen Beweis für stetiges $Z$ (Beweisidee: man betrachte, analog zu hier $z=1$, dasjenige $z$, für das die Varianz maximal ist, $z^\ast \coloneqq \underset{z}{argmax} Var(Y|x,z)$.)\\
Ich finde das Ergebnis spannend, aber nicht so leicht zu durchschauen. Die wahre Varianz von $Var(Y|x,z=1)$ wird natürlich nicht dadurch kleiner, dass ich $Z$ ignoriere! :) Aber, wie in den Beispiel-Szenarien mit dem linearen Modell, die jetzt im Appendix \ref{sec:app.omitted variables} sind, sind Unsicherheitsquantifikationen, die auf $Var(Y|x)$ aufbauen einfach "off" und es kommt zu undercoverage (im obigen Beispiel: für $z=1$) und overcoverage (im obigen Beispiel: für $z=0$).\\
%Das $Var(Y|x,z)$, das im ersten Integranden steht, ist nicht dasselbe $Var(Y|x,z)$, weil im Integranden $z$ kein fester Wert ist, sondern ein "Platzhalter" fuer eine Variable bzgl. der integriert wird.\\
2. sehe ich nicht wie das Resultat mit den Annahmen dieses Absatzes zusammenhaengt: diese Varianzformel gilt doch allgemein und nicht nur die beiden Unabhängigkeiten? Dann würde ich das lieber weiter oben schreiben, als generlles Resultat, anstatt hier in einem der spezifischen Szenarien.\\
3. geklaert, weggefallen, danke MS!\\%sehe ich nicht, wieso die rechte Seite von \eqref{eq:varincrease} die Varianz $ Var(Y|x)$ ist
4. Im Gegensatz zu späteren subsections, haben $Var$ und $E$ hier keine Tiefindizes, die zeigen würden, bzgl. was man hier Erwartungswerte hat.  einheitliche Notation wäre schon gut, wenn nix dagegen spricht.} 


==> 5-data-uncertainty/missing-data-cutout.tex <==
The pertinent literature (\cite{little2019statistical}) recognises three mechanisms or types of missingness. \emph{Missing completely at random}, MCAR, denotes the case where the missing and the observed units do not differ systematically or, put differently, where the propensity of missingness is independent of both, observed and missing values. With MCAR, a naive complete-case analysis provides unbiased results. But the complete-case analysis, which is what most standard software packages do by default, is not efficient, meaning that the \add{epistemic} uncertainty is increased. 
Data is \emph{missing at random}, MAR, when the propensity of missingness depends only on observed but not on missing values, i.e., when, after conditioning on the observed information, the variable with the missing values has the same distribution among the observed units as among the units without values. In this situation, a complete case analysis may lead to biased results, if the missingness occurs in the input variables $X$. To see this, let $R^{(i)}$ be an indicator variable which takes value $1$ if $x^{(i)}$ is observed and $0$ otherwise. Note that the complete data consist of $(y^{(i)},x^{(i)},R^{(i)}=1)$ so that any model trained on the complete data aims to learn the model $f_{Y|X,R}(y|x,R=1)$. Simple %\pat{die Umformungen waren simpel, aber fuer mich warens ca. 4 Umformungen, die gebraucht habe, sprich Ergebnis nicht sofort ersichtlich. $\rightarrow$ Appendix?} 
calculations yield
\begin{align*}
    f_{Y|X,R}(y|x,R=1) = \frac{\Prob (R=1 | y , x )}{\Prob(R=1 | x )} f_{Y|X}(y|x)
 = \underbrace{\frac{\Prob (R=1 | y )}{\Prob(R=1 | x)}}_{\mbox{ Bias }} f_{Y|X}(y|x),
    \tag{S}
    \label{eq:S}
 \end{align*}
 where $P(R=1 | x ) = \int P(R=1|y) f_{Y|X}(y|x) dy $. Consequently, we can omit the conditioning on $X$ in the probability for $R $ \comment{due to the assumed missing at randomness.}{PS: Das glaube ich ehrlich gesagt nicht: MAR heisst ja nur, dass man dafuer korrigieren kann, aber hier ist noch nix korrigiert. Ausserdem ist ja in unserem allgemeinen Setup gar nicht festgelegt, ob missigness in $x$ vorliegt oder in $y$ oder in beidem und MAR stellt ja auf beobachtete/unbeobachtete Variablen ab und nicht auf features/labels. $X$ beinhaltet potentiell auch nichtbeobachtete Information und umgekehrt kann beobachtete Information $Y$ umfassen.\\
 Was im Moment drin steht ist die Behauptung dass $\Prob (R=1)$ konstant ist für alle $x$ -- und das ist nicht identisch mit MAR. Das waere tendenziell eher MCAR (wieder mit der Einschraenkung, dass wir in unserem framework ja nicht gesagt haben, ob missingness in y, x, oder beidem und es darum nicht perfekt sauber passt.) MAR bedeutet:\\
 $\Prob (R=1 | (x,y)_{\text{miss}},(x,y)_{\text{obs}}) = \Prob (R=1 | (x,y)_{\text{obs}})$, siehe Little \& Rubin (2002, S. 16, 2. Gleichung).} \textcolor{red}{GK: Ist korrigiert. Man kann auf Little verweisen, aber wir sollten $Y$ univariat lassen und wir sagen ja, dass wir missing in $X$ annehmen.\\}
\pat{\textbf{Antwort}: Ich bin mir leider immer noch unsicher, sorry. Ja, dass wir missing in $X$ annehmen, steht da, und univariates $Y$ auf jeden Fall. Oder war univariates $X$ gemeint? Jedenfalls:\\
a. reden wir dann automatisch, durch die Hintertür nur noch über item nonresponse und haben unit nonresponse plötzlich ausgeklammert (denn unit non response = es fehlt alles, inkl. y).\\
b. auch wenn $Y$ nie fehlt, sondern nur $X$, kann $\Prob(R=1|y,x)$ trotzdem noch von $Y$ abhängen. typischer Fall: $Y$ Einkommen, $X$ sind features die Einkommen erklären können. Je höher $Y$, desto höher die Wahrscheinlichkeit von Nonrespone, und das auch bedingt auf $X$. Anders ausgedrückt, in linearem Modell: das Residuum  $\epsilon = Y - \beta X$ ist noch mit $R$ korreliert selbst wenn schon für $X$ kontrolliert hat. \\
c. wir unterscheiden nicht in $x_{\text{obs}},x_{\text{obs}}$ und dies differenziert ja genau MAR und NMAR. Die Formel wird dadurch nicht falsch, aber die Frage ist dann, warum \eqref{eq:S} in Fall MAR drin steht und nicht übergeordnet vor allen Fällen. Dann könnte man eben sagen: 1) MCAR: eh kein Problem, der Quotient ist 1, kein Bias. 2) MAR: Bias. Traditionelle Verfahren können den Bias schätzen bzw korrigieren, z.B. via Gewichtung oder Imputation. Und dann auf die epistemic uncertainty des Korrekturmodells eingehen. Verbesserung der Prädiktion(sunsicherheit), in dem missingness Indikator berücksichtigt wird (sh unten). 3. NMAR: Traditionelle Verfahren können den Bias nicht schätzen.}
 
 \pat{1. Warum $R$ statt $Z$? %Wenn $Z$ frei ist, warum nehmen wir dann nicht $Z$ her anstatt eine neue Variable $R$ einzuführen? Sind missing data anders als unser framework \eqref{eq:true_xyz}--\eqref{eq:datpred} und wir wollen $Z$ darum absichtlich vermeiden? Dann lohnt es sich, explizit zu sagen, dass unser framework hier nicht passt. Ein klarer Unterschied: $Z$ war immer unobserved, aber der Indikator $R$ ist ja schon beobachtet.  
 2. Die Behauptung " any model trained on the complete data aims to learn the model $f_{Y|X,R}(y|x,R=1)$." finde ich nicht trivial und das Wort "aims" insbesondere. Genau an der Stelle steckt für mich ein Großteil der Erkenntnisse drin? Denn tradtionelle Missing Data Verfahren wollen genau das nicht, sondern sie wollen einen "population average Effekt" lernen, wobei der population average die Integration über die response propensity bedeutet. Wollen ML Verfahren das auch? Oder wollen sie einbeziehen, dass die respondents tendenziell anders sind als die nonrespondents? Falls ja, ist man wieder in sowas wie omitted variable Situation: die response propensity $Z$ ist unbeboachtet und für unterschiedliche Werte von $Z$ bekommt unterschiedlich gute predictions. 3. die Imputation/Gewichtung und der damit einher gehende trade-off der zwei epistemischen Unsicherheiten (eine im ML Modell und eine im Modell für die Imputation/Gewichtung) ist nicht thematisiert; das ist für mich ein wichtiger Bezug zum Thema der Arbeit.}
 An example is, if $Y$  is the opinion about a product bought on a retailer's webpage and $X$ is the text accompanying the opinion. We may find that in case of a positive opinion $Y$, the customer is less likely to accompany this opinion by a text $X$. In this case, learning the sentiment $Y $ from the text $X $ based on the data at hand will lead to biased models. 

Finally, data are \emph{missing not at random}, MNAR, when the propensity of missingness (also) depends on the missing values. In this case, any data analysis will be heavily biased. \pat{naja, je nach Staerke. Es gibt auch papers die zeigen dass complete case analysis bei MNAR in ihrem Szenario nix schlimmes anrichtet.} 

\highlight{check cross-references below, as far as they are still needed:}
A higher-level discussion of the consequences of the training data not being representative of the target population in deployment can be found in section~\ref{subsec:deployment}. MAR and MNAR are two reasons for such a discrepancy. In this subsection, \ref{subsec:missing.data}, we highlight aspects that are specific to missing data.

%There are four groups of methods for missing data \citep[ch.~1.4]{little.rubin.2002.missing.data.book} which, as in the section on errors in $X$, we will call correction methods: complete-case analysis, weighting-based procedures, imputation-based procedures (which fill in the missing values with predictions), and methods based on statistical models (e.g., likelihood and Bayes). The latter is not of particular practical relevance to most machine learning. In our experience, weighting is more used for unit nonresponse and imputation more for item nonresponse; they both help to repair data suffering from MAR.


%\subsubsection*{Consequences}
Besides the mentioned bias problems, missing data lead to further problems. First, missingness reduces the size of the available data 
%sample for unit nonresponse and for item nonresponse data 
analysed with a complete-case approach. Hence, any uncertainty that could be reduced with increased sample size suffers. The effect can be quite dramatic for item nonresponse: even if the overall rate of missing values among all %\replace{field}
{cell}s low, in settings with very many features the number of observations with at least one missing %\replace{field}
{cell} can be relatively high. \pat{Can be briefly shown in a figure or table.} %\cg{again: fields vs. cells} 
This makes complete-case analysis, while convenient, potentially very inefficient for uncertainty reduction compared to, e.g., imputation. 
%However, what may seem like aleatoric uncertainty is only caused by inefficient use of the available information. By employing appropriate methodology and without any new instances, variables, or other form of information at all, uncertainty can be reduced, again showing that what one considers aleatoric can be highly dependent on one's decisions for the data analysis (here: whether to correct for missingness or not).

Second, replacing missing values via imputation is done \cg{"is done" is a imprecise phrasing, what is meant exactly? "adds aleatoric uncertainty"?} with aleatoric uncertainty: the missing value is not known exactly but predicted with uncertainty. Faithful uncertainty quantification accounts for this by using multiple imputation\footnote{
	For each variable, a model is estimated that predicts the variable based on the other variables. This model is used to predict the value where it is missing. Replacing a missing value with the predicted value ignores uncertainty. Instead, multiple data sets are created: say $K=10$ and for each dataset, instead of just the prediction, a random draw from the predictive distribution (of this instance) is drawn. The $K$ datasets are each analysed as usual. The $K$ results are then combined. In parametric models, the mean of the $K$ parameter estimates is the eventual estimate. Sampling variability and imputation uncertainty are accounted for as well.
} 
or resampling methods to estimate the additional uncertainty introduced by the imputation. For predictive modelling, this has two implications. 
i) We can also use these tools to quantify the additional predictive uncertainty introduced by having to impute missing values. Local estimation uncertainty, and thus predictive uncertainty, will likely be higher in areas of the $X$ space with more missing values.
ii) Of two predictions with the same value $x_0$, the prediction that is based on having imputing $x_0$ is more uncertain than the one based on an actually observed $x_0$.

Third, the models employed for imputation or weighting are, as any model, susceptible to %sampling error and misspecification errors. 
model uncertainty and estimation uncertainty. On the latter, the increased use of machine learning has helped.\footnote{
	This is not quite as easy for multiple imputation as it requires a draw from a predictive distribution. Machine learning ensembles are a way to replace what in classical statistical models is supplied by distributional assumptions. (REF needed?)
} 
In our experience, the epistemic uncertainty of the correction methods is often forgotten in both, traditional statistical modelling and machine learning based prediction. The epistemic uncertainty may be quite high when we do not have many observations for learning the correction models well, or when there are complex relationships, or when we need to rely on outside information.

Fourth, there is a trade-off. On the one hand, missingness correction methods (weighting and imputation) can improve the epistemic uncertainty of our trained model $\hat{p}(y|x)$ through more and better data. On the other hand, they are themselves subject to epistemic uncertainty which then increases epistemic uncertainty in $\hat{p}(y|x)$. The trade-off does not only depend on these two types of epistemic uncertainty, but also on the aleatoric uncertainty in the correction methods: how well can nonresponse be predicted for weighting or how well can the missing values be predicted for imputation.


==> figures/KL_decreasing_ridge.tex <==
% Created by tikzDevice version 0.12.4 on 2023-03-13 14:46:02
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,361.35);
\begin{scope}
\path[clip] ( 34.44,275.34) rectangle (199.17,339.51);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.54,337.13) --
	( 44.45,335.67) --
	( 48.36,333.74) --
	( 52.27,331.19) --
	( 56.18,329.40) --
	( 60.10,327.18) --
	( 64.01,324.26) --
	( 67.92,323.79) --
	( 71.83,320.55) --
	( 75.74,319.27) --
	( 79.65,317.98) --
	( 83.56,315.21) --
	( 87.47,314.03) --
	( 91.38,311.47) --
	( 95.29,311.03) --
	( 99.21,311.14) --
	(103.12,311.27) --
	(107.03,312.92) --
	(110.94,321.43) --
	(114.85,336.94) --
	(118.76,333.57) --
	(122.67,301.23) --
	(126.58,284.52) --
	(130.49,278.22) --
	(134.40,277.72) --
	(138.32,278.41) --
	(142.23,281.96) --
	(146.14,286.66) --
	(150.05,290.71) --
	(153.96,294.37) --
	(157.87,297.23) --
	(161.78,299.46) --
	(165.69,300.35) --
	(169.60,301.94) --
	(173.51,303.99) --
	(177.43,305.52) --
	(181.34,308.07) --
	(185.25,308.41) --
	(189.16,309.01) --
	(193.07,311.05);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,361.35);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98,275.34) -- (195.42,275.34);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98,275.34) -- ( 38.98,271.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 78.09,275.34) -- ( 78.09,271.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (117.20,275.34) -- (117.20,271.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.31,275.34) -- (156.31,271.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (195.42,275.34) -- (195.42,271.14);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 38.98,260.22) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 78.09,260.22) {50};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (117.20,260.22) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (156.31,260.22) {150};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (195.42,260.22) {200};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 34.44,275.34) --
	(199.17,275.34) --
	(199.17,339.51) --
	( 34.44,339.51) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,240.90) rectangle (216.81,361.35);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.84] at (116.80,347.53) {\bfseries $E_X\left\{ KL( f(\cdot|X), p(\cdot|X; \hat{\theta}_{pen}))\right\}$, Eq.(12)};
\end{scope}
\begin{scope}
\path[clip] ( 34.44,154.89) rectangle (199.17,219.06);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.54,216.68) --
	( 44.45,215.96) --
	( 48.36,215.18) --
	( 52.27,214.33) --
	( 56.18,213.49) --
	( 60.10,212.62) --
	( 64.01,211.68) --
	( 67.92,210.74) --
	( 71.83,209.72) --
	( 75.74,208.77) --
	( 79.65,207.59) --
	( 83.56,206.50) --
	( 87.47,205.35) --
	( 91.38,203.99) --
	( 95.29,202.69) --
	( 99.21,201.09) --
	(103.12,199.63) --
	(107.03,198.03) --
	(110.94,196.14) --
	(114.85,194.20) --
	(118.76,192.17) --
	(122.67,189.74) --
	(126.58,187.10) --
	(130.49,184.12) --
	(134.40,180.62) --
	(138.32,176.66) --
	(142.23,171.75) --
	(146.14,166.07) --
	(150.05,160.29) --
	(153.96,157.41) --
	(157.87,157.27) --
	(161.78,157.27) --
	(165.69,157.27) --
	(169.60,157.27) --
	(173.51,157.27) --
	(177.43,157.27) --
	(181.34,157.27) --
	(185.25,157.27) --
	(189.16,157.27) --
	(193.07,157.27);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,361.35);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98,154.89) -- (195.42,154.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98,154.89) -- ( 38.98,150.69);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 78.09,154.89) -- ( 78.09,150.69);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (117.20,154.89) -- (117.20,150.69);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.31,154.89) -- (156.31,150.69);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (195.42,154.89) -- (195.42,150.69);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 38.98,139.77) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 78.09,139.77) {50};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (117.20,139.77) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (156.31,139.77) {150};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (195.42,139.77) {200};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 34.44,154.89) --
	(199.17,154.89) --
	(199.17,219.06) --
	( 34.44,219.06) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,120.45) rectangle (216.81,240.90);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.84] at (116.80,227.08) {\bfseries Eq. (13)};
\end{scope}
\begin{scope}
\path[clip] ( 34.44, 34.44) rectangle (199.17, 98.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.54, 36.82) --
	( 44.45, 37.31) --
	( 48.36, 37.78) --
	( 52.27, 38.19) --
	( 56.18, 38.75) --
	( 60.10, 39.26) --
	( 64.01, 39.70) --
	( 67.92, 40.62) --
	( 71.83, 41.09) --
	( 75.74, 41.87) --
	( 79.65, 42.90) --
	( 83.56, 43.53) --
	( 87.47, 44.55) --
	( 91.38, 45.52) --
	( 95.29, 46.84) --
	( 99.21, 48.60) --
	(103.12, 50.21) --
	(107.03, 52.28) --
	(110.94, 56.03) --
	(114.85, 61.22) --
	(118.76, 62.76) --
	(122.67, 58.98) --
	(126.58, 58.52) --
	(130.49, 60.51) --
	(134.40, 64.22) --
	(138.32, 68.66) --
	(142.23, 74.70) --
	(146.14, 81.81) --
	(150.05, 88.91) --
	(153.96, 92.77) --
	(157.87, 93.49) --
	(161.78, 93.93) --
	(165.69, 94.11) --
	(169.60, 94.42) --
	(173.51, 94.83) --
	(177.43, 95.13) --
	(181.34, 95.64) --
	(185.25, 95.71) --
	(189.16, 95.83) --
	(193.07, 96.23);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,361.35);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98, 34.44) -- (195.42, 34.44);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 38.98, 34.44) -- ( 38.98, 30.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 78.09, 34.44) -- ( 78.09, 30.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (117.20, 34.44) -- (117.20, 30.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.31, 34.44) -- (156.31, 30.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (195.42, 34.44) -- (195.42, 30.24);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 38.98, 19.32) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 78.09, 19.32) {50};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (117.20, 19.32) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (156.31, 19.32) {150};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (195.42, 19.32) {200};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 34.44, 34.44) --
	(199.17, 34.44) --
	(199.17, 98.61) --
	( 34.44, 98.61) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,120.45);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.84] at (116.80,106.63) {\bfseries Eq. (14)};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (116.80,  2.52) {p};
\end{scope}
\end{tikzpicture}

